Hopf-Frobenius Algebras and a Simpler Drinfeld Double

The zx-calculus and related theories are based on so-called interacting Frobenius algebras, where a pair of dagger-special commutative Frobenius algebras jointly form a pair of Hopf algebras. In this setting we introduce a generalisation of this structure, Hopf-Frobenius algebras, starting from a single Hopf algebra which is not necessarily commutative or cocommutative. We provide a few necessary and sufficient conditions for a Hopf algebra to be a Hopf-Frobenius algebra, and show that every Hopf algebra in the category of finite dimensional vector spaces is a Hopf-Frobenius algebra. In addition, we show that this construction is unique up to an invertible scalar. Due to this fact, Hopf-Frobenius algebras provide two canonical notions of duality, and give us a "dual" Hopf algebra that is isomorphic to the usual dual Hopf algebra in a compact closed category. We use this isomorphism to construct a Hopf algebra isomorphic to the Drinfeld double, but has a much simpler presentation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{150}
\providecommand{\publicationstatus}{Bob Coecke and Mathew Leifer (Eds.):\\ Quantum Physics and Logic 2019 (QPL)\\
EPTCS 318, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.318.10}{10.4204/EPTCS.318.10}}
\pdfoutput=1


==> front-matter.tex <==

%%%%%%%%%%%%%% this is a hack for the EPTCS style's limitations

\RequirePackage{array}  %%% needed for EPTCS authors hack

\newenvironment{authors}[1]%
  {\begingroup
   \newcommand\estyle{}%
   \renewcommand\institute[1]%
     {\\\multicolumn{#1}{@{}c@{}}{\scriptsize\begin{tabular}[t]{@{}>{\footnotesize}c@{}}##1\end{tabular}}}%
   \renewcommand\email[1]%
     {\gdef\estyle{\footnotesize\ttfamily}\\##1\gdef\estyle{}}
   \begin{tabular}[t]{@{}*{#1}{>{\estyle}c}@{}}
  }%
  {\end{tabular}%
   \endgroup
  }
%%%%%  END HACK %%%%%%%%%%%%%%%%%%%%%%%%%%%% 


\title{Hopf-Frobenius Algebras and a Simpler Drinfeld Double}

\author{  
\begin{authors}{2}
Joseph Collins$^{1}$ & Ross Duncan$^{1,2}$
\email{joseph.collins@strath.ac.uk & ross.duncan@strath.ac.uk}
\institute{${}^1$Department of Computer and Information Sciences\\
University of Strathclyde\\
26 Richmond Street, Glasgow, United Kingdom}
\institute{${}^2$Cambridge Quantum Computing Ltd\\
9a Bridge Street, Cambridge, United Kingdom}
\end{authors}
}
\def\titlerunning{Hopf-Frobenius Algebras and a Simpler Drinfeld Double}
\def\authorrunning{J. Collins \& R. Duncan}


